Quality of Control Assessment for Tactile Internet based Cyber-Physical Systems

We evolve a methodology and define a metric to evaluate Tactile Internet based Cyber-Physical Systems or Tactile Cyber-Physical Systems (TCPS). Towards this goal, we adopt the step response analysis, a well-known control-theoretic method. The adoption includes replacing the human operator (or master) with a controller with known characteristics and analyzing its response to slave side step disturbances. The resulting step response curves demonstrate that the \textit{Quality of Control} (QoC) metric is sensitive to control loop instabilities and serves as a good indicator of cybersickness experienced by human operators. We demonstrate the efficacy of the proposed methodology and metric through experiments on a TCPS testbed. The experiments include assessing the suitability of several access technologies, intercontinental links, network topologies, network traffic conditions and testbed configurations. Further, we validate our claim of using QoC to predict and quantify cybersickness through experiments on a teleoperation setup built using Mininet and VREP.

==> readMe.tex <==
What is not taken care -
** 

-- Remove all references to haptic-in-video signal in figures ? See all figures and rearrange accordingly
3rd OCtober 201

reason for display driver delay - remove

place sensors on figure

operator side implementation trade off smaller delta

Why settling time and undershoot is not accounted

Packet drops ? in Figure 9

Scaled haptic response ?

Recall that typo in step response ...

Factoring in effect of data packet size ... last line packet drop change to packet corrup or error

Table for literature. ChANGE GROUP TO DEF

lITERATURE SECTION LAST FEW LINES ARE JUMBLED - BOTH DELTA AND TR DEPENDE ...

Also, review the evaluation model, and replace any occurance of haptic-in visual or kinematic-haptic-video to kinematic-haptic

13 Sep 2019

Comments from TVP:

- Cybersickness canresult  in  general  discomfort,  headache,  stomach  awareness,nausea, fatigue and drowsiness in humans and deter the humanoperators from prolonged use of the teleoperation system. (Give citation)

- However,  realizing  tactileinternet is only one part, significant research concerning designand  evaluation  is  necessary  also  in  building  the  optimizedhardware,  algorithms  and  protocols  that  accompany  a  TCPSapplication.
TVP - State that even if one component is tactile ready, it doesn't mean that the end system is TCPS ready.

- Differentiate between Cybersickness and control loop quality (Does 1 imply other ?)

- Define if we are testing end-end system and sub system.

- Define +ve synchrnoziation error

- Define the case with mpeg where audio and video and transmitted seperately 

- What do you mean by feedback latency (does it include network and non-netwworking latencies)

- Control loop for evaluation. Why evaluating all control loops is cumbersome and resource consuming.

- What is the practical case of Application-1 and Application-2

>>>>>>>
28th Aug
-- QoC is used whenever we are referring to Quality of Control. \overline(QoC) is used to present measurement results.
-- replace X in figures to x
- Change plant state variable from x to s ?
- Change g to fraction
- Change QoC to QoC (g)
-- Replace QoC to QoC (g) in QoC performance curve ?

1. Footnote ?

2. Discussion:Haptic feedback can be of two types tactilefeedback and kinesthetic feedback. In the paper, when we referto  haptic  feedback,  we  intend  tactile  feedback.  Although  theTCPS evaluation model could be extended to incorporate thebilateral nature of kinesthetic feedback, in the current version,we did not invest our time and effort in this direction.

3. x<Xunits ??? 1cm ??





<<<<<<<
--Let us now discuss the RTT requirements for different TCPScontrol  loops  to  avoid  cybersickness.  

-- Rewrite our contribution.

-- Haptic feedback/ Haptic Data

Section:4 QoC
-- Observe that, with 20% limit, the overshoots and steady state error for good response curves should be less than ... and ..., respectively. In particular, peaks of good response curves should be less than ... .
-- implies a potentially smaller t_d, i.e., a smaller RTT_{}, and hence a better quality TCPS. 

-- Not footnote ?? "Observe that if we restrict the human operator’s maximum hand ..."

Add citations for Introduction

(1) Our contribution ?
(2) Give section overview in Section-I end.


Change/rewrite the definitions of QoC

QoC in a relaxed setting ...

Add Joydeep
Change tilte
Specify that it is a extension of conference ?
Change abstract and summary ?
Add a section on QoC in a relaxed setting.




** Give reference to SECON paper

----
QoC in Real Time:

https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=4042685

https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=4700443

https://old.liu.se/elliit/artiklar-3/1.741925/AmirAminifar.pdf

https://infoscience.epfl.ch/record/231419/files/DT_DTSI-2017-03-0067.R1_Aminifar.pdf

http://www.cis.upenn.edu/~lee/04cis700/papers/CEBA02.pdf

https://link.springer.com/content/pdf/10.1007%2Fs11241-011-9133-x.pdf


------
#2 Determining network bounds:
Let’s say the application requires a Vmax = v m/s
Now input this value to the model and required reliability value ‘g’ 
Also input link latency and jitter
The model should give bounds on the network parameter packet drop.

#4 Discuss QoC papers in RTSS literature and how they are different from our definition.

#5 Can we experimentally determine the QoC performance curve and use it for comparing the performance of real systems ?. This could be added in the experimental section.

#6 Experiment with IEEE 802.11ax (supported by ns3) suggested by reviewer. ?

